A Logic-Independent IDE

The author's MMT system provides a framework for defining and implementing logical systems. By combining MMT with the jEdit text editor, we obtain a logic-independent IDE. The IDE functionality includes advanced features such as context-sensitive auto-completion, search, and change management.

==> eptcsdata.tex <==
\providecommand{\firstpage}{48}
\providecommand{\publicationstatus}{C. Benzm\"uller and B. Woltzenlogel Paleo (Eds.):\\ 
Eleventh Workshop on User Interfaces for Theorem Provers (UITP 2014)\\
EPTCS 167, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.167.7}{10.4204/EPTCS.167.7}}
\pdfoutput=1

